Changes in European Solidarity Before and During COVID-19: Evidence from a Large Crowd- and Expert-Annotated Twitter Dataset

We introduce the well-established social scientific concept of social solidarity and its contestation, anti-solidarity, as a new problem setting to supervised machine learning in NLP to assess how European solidarity discourses changed before and after the COVID-19 outbreak was declared a global pandemic. To this end, we annotate 2.3k English and German tweets for (anti-)solidarity expressions, utilizing multiple human annotators and two annotation approaches (experts vs.\ crowds). We use these annotations to train a BERT model with multiple data augmentation strategies. Our augmented BERT model that combines both expert and crowd annotations outperforms the baseline BERT classifier trained with expert annotations only by over 25 points, from 58\% macro-F1 to almost 85\%. We use this high-quality model to automatically label over 270k tweets between September 2019 and December 2020. We then assess the automatically labeled data for how statements related to European (anti-)solidarity discourses developed over time and in relation to one another, before and during the COVID-19 crisis. Our results show that solidarity became increasingly salient and contested during the crisis. While the number of solidarity tweets remained on a higher level and dominated the discourse in the scrutinized time frame, anti-solidarity tweets initially spiked, then decreased to (almost) pre-COVID-19 values before rising to a stable higher level until the end of 2020.

==> tables/ensembling.tex <==
\begin{table}[!htb]
    \centering
    \begin{tabular}{c|c|cc}
     \toprule
     & &  MBERT & XLM-R\\
    &Ensembling& dev set& test set\\
    \midrule
    \multirow{2}{*}{E} & 3 models & 0.758& 0.741\\
    & all models & 0.771& 0.783\\ % ensemble of 10
    \midrule
    \multirow{2}{*}{E+C} & 3 models & 0.790 & 0.802\\
    & all models & 0.824& 0.834\\ % ensemble of 9
    \bottomrule
    \end{tabular}
    \caption{Macro-F1 scores for ensembling different %number of 
    models. Top-3 models are determined by dev score.}
    \label{table:improvement with ensembling}
\end{table}

==> tables/tablepart_baselines.tex <==
\begin{table}[!htb]
    \centering
    \begin{tabular}{c|cc|cc}
     \toprule
         &  \multicolumn{2}{|c|}{MBERT} & \multicolumn{2}{|c}{XLM-R}\\     & dev set & test set & dev set & test set\\\midrule
         E &  0.650 & 0.557 & 0.657 & 0.656 \\ 
         E+C & 0.660 & 0.634 & 0.650 & 0.648 \\
         \bottomrule
    \end{tabular}
    \caption{F1 scores for MBERT and XLM-R models on the development and the test set. ``E'' means that the training instances are only sampled from expert annotations. ``E+C'' means that the training samples come from expert and crowd annotations.}
    \label{table:improvement_with_crowd_annotations}
\end{table}

